Precision Anti-Cancer Drug Selection via Neural Ranking

Personalized cancer treatment requires a thorough understanding of complex interactions between drugs and cancer cell lines in varying genetic and molecular contexts. To address this, high-throughput screening has been used to generate large-scale drug response data, facilitating data-driven computational models. Such models can capture complex drug-cell line interactions across various contexts in a fully data-driven manner. However, accurately prioritizing the most sensitive drugs for each cell line still remains a significant challenge. To address this, we developed neural ranking approaches that leverage large-scale drug response data across multiple cell lines from diverse cancer types. Unlike existing approaches that primarily utilize regression and classification techniques for drug response prediction, we formulated the objective of drug selection and prioritization as a drug ranking problem. In this work, we proposed two neural listwise ranking methods that learn latent representations of drugs and cell lines, and then use those representations to score drugs in each cell line via a learnable scoring function. Specifically, we developed a neural listwise ranking method, List-One, on top of the existing method ListNet. Additionally, we proposed a novel listwise ranking method, List-All, that focuses on all the sensitive drugs instead of the top sensitive drug, unlike List-One. Our results demonstrate that List-All outperforms the best baseline with significant improvements of as much as 8.6% in hit@20 across 50% test cell lines. Furthermore, our analyses suggest that the learned latent spaces from our proposed methods demonstrate informative clustering structures and capture relevant underlying biological features. Moreover, our comprehensive empirical evaluation provides a thorough and objective comparison of the performance of different methods (including our proposed ones).

==> tables/abbv.tex <==
\renewcommand{\arraystretch}{1.1}

\begin{table}[h]
\centering
\caption{List of Abbreviations}
\label{tbl:abbv}

\begin{threeparttable}
\begin{tabular}{
 	@{\hspace{2pt}}l@{\hspace{2pt}}
 	@{\hspace{2pt}}p{12cm}@{\hspace{2pt}}
	}
	\toprule
	Abbreviation & Meaning \\         
	\midrule
        \RankNet & \underline{Pair}wise learning to rank jointly with \underline{Push} and drug \underline{C}lassification \\
        \ListNet & \underline{List}wise learning to rank for top-\underline{One} sensitive drug selection \\
        \SelNet & \underline{List}wise learning to rank for \underline{All} sensitive drug selection \\
	\GeneAE & \underline{Gene} \underline{A}uto-\underline{E}ncoder \\
	\GeneE & \underline{Gene} \underline{E}ncoder \\
	\GeneD & \underline{Gene} \underline{D}ecoder \\
	\DrugE  & Fully connected neural network to learn \underline{Drug} \underline{E}mbedding \\
	\csimB & Average pairwise \underline{c}ell line \underline{sim}ilarities computed from embeddings out of the best \underline{B}aseline \\
	\csimM & Average pairwise \underline{c}ell line \underline{sim}ilarities computed from embeddings out of the best-proposed \underline{M}ethod \\
	\csimS & Average pairwise \underline{c}ell line \underline{sim}ilarities computed from drug \underline{R}esponse profiles \\
	\dsimB & Average pairwise \underline{d}rug similarities computed from embeddings out of the best \underline{B}aseline \\
	\dsimM & Average pairwise \underline{d}rug similarities computed from embeddings out of the best-proposed \underline{M}ethod \\
	\dsimS  & Average pairwise \underline{d}rug similarities computed from cell \underline{S}ensitivity profiles \\
        
       \bottomrule
   
         \end{tabular}
\end{threeparttable}

\end{table}

==> tables/overall_nc_prism.tex <==
\begin{table}[h!]
\centering
\caption{Overall Comparison for PRISM in LCO validation}
\label{tbl:overall_nc_prism}

  \begin{threeparttable}
      \begin{tabular}{
          @{\hspace{2pt}}l@{\hspace{1pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
          %@{\hspace{3pt}}r@{\hspace{3pt}}
	  %@{\hspace{3pt}}r@{\hspace{3pt}}
          }
          \toprule
	  model  & AP@1 &  AP@3   & AH@3   & AP@5   & AH@5   & AP@10  & AH@10  
	  & AP@20  & AH@20   & AP@40  & AH@40   & AP@60  & AH@60  \\ %& sCI    & CI     \\
	  \midrule
	%\cclerank & 0.9977 & 0.9980 & 2.9783 & 0.9962 & 4.9327 & 0.9897 & 9.7734 
	%& 0.9799 & 18.9532 & 0.9501 & 33.7018 & 0.9285 & 38.9641 & 0.7579 & 0.7960 \\
	%\cclerank & 0.9977 & 0.9976 & 2.9803 & 0.9963 & 4.9418 & 0.9908 & 9.7924 
	%& 0.9811 & 18.9552 & 0.9503 & 33.6161 & 0.9278 & 38.8026 & 0.7614 & 0.7996 \\
	%\cclerank & 0.9977 & 0.9980 & 2.9803 & 0.9965 & 4.9437 & 0.9907 & 9.7924 
	%& 0.9811 & 18.9582 & 0.9505 & 33.6815 & 0.9286 & 38.8354 & 0.7605 & 0.7988 \\
	\cclerank & 0.9977\rlap{*} & 0.9980\rlap{*} & 2.9803\rlap{*} & 0.9965\rlap{*} & 4.9437\rlap{*} & 0.9907 & 9.7924 
	& 0.9811 & 18.9582 & 0.9505 & 33.6815 & 0.9286 & 38.8354\\ % & 0.7605 & 0.7988 \\
	%\cclerank & 0.9977 & 0.9976 & 2.9803 & 0.9963 & 4.9418 & 0.9908 & 9.7924 
	%& 0.9811 & 18.9552 & 0.9503 & 33.6161 & 0.9278 & 38.8026 & 0.7614 & 0.7996 \\
	%\cclerank & 0.9977 & 0.9976 & 2.9803 & 0.9963 & 4.9418 & 0.9908 & 9.7924 
	%& 0.9811 & 18.9552 & 0.9503 & 33.6161 & 0.9278 & 38.8026 & 0.7614 & 0.7996 \\
	\cclerank & 0.9977 & 0.9976 & 2.9803 & 0.9963 & 4.9418 & 0.9908\rlap{*} & 9.7924\rlap{*} 
	& 0.9811\rlap{*} & 18.9552 & 0.9503 & 33.6161 & 0.9278 & 38.8026 \\ %& 0.7614 & 0.7996 \\
	\cclerank & 0.9936 & 0.9950 & 2.9586 & 0.9914 & 4.9200 & 0.9849 & 9.6878 
	& 0.9741 & 19.0166\rlap{*} & 0.9516 & 35.0500 & 0.9232 & 45.8071 \\  % & 0.7220 & 0.5935 \\
	\cclerank  & 0.9936 & 0.9961 & 2.9760 & 0.9941 & 4.9263 & 0.9870 & 9.7005 
	& 0.9757 & 18.9866 & 0.9527\rlap{*} & 35.0051 & 0.9239 & 45.7952 \\ % & 0.7269 & 0.7222 \\
	\cclerank & 0.9936 & 0.9943 & 2.9630 & 0.9918 & 4.9244 & 0.9850 & 9.6987 
	& 0.9743 & 19.0097 & 0.9517 & 35.0608\rlap{*} & 0.9234 & 45.7869 \\ %& 0.7224 & 0.5940 \\
	\cclerank  & 0.9977 & 0.9972 & 2.9783 & 0.9959 & 4.9413 & 0.9899 & 9.7842 
	& 0.9805 & 18.9497 & 0.9503 & 33.7126 & \textbf{0.9287}\rlap{*}  & 38.8932 \\ %& 0.7591 & 0.7975 \\
	\cclerank  & 0.9936 & 0.9953 & 2.9737 & 0.9939 & 4.9240 & 0.9865 & 9.6917 
	& 0.9750 & 19.0031 & 0.9520 & 35.0117 & 0.9233 & \textbf{45.8240}\rlap{*} \\ %& 0.7234 & 0.6785 \\
	%\cclerank &  0.9977 & 0.9976 & 2.9803 & 0.9963 & 4.9418 & 0.9908 & 9.7924 
	%& 0.9811 & 18.9552 & 0.9503 & 33.6161 & 0.9277 & 38.8171 \\ %& 0.7615\rlap{*} & 0.7996\rlap{*} \\
	%\cclerank & 0.9977 & 0.9976 & 2.9803 & 0.9963 & 4.9418 & 0.9908 & 9.7924 & 0.9811 & 18.9552 & 0.9503 & 33.6161 & 0.9278 & 38.8026 & 0.7614 & 0.7996 \\
	\hline
	%%
	\deepcdr & 0.9978 & 0.9984 & 2.9715 & 0.9955 & 4.9329 & 0.9900 & 9.7774 
	& 0.9783 & 18.8535 & 0.9491 & 34.3966 & 0.9190 & 43.8519 \\ %& 0.7435 & 0.7996 \\
	\hline
	%%
	%\RankNet & 0.9987 & 2.9777 & 0.9963 & 4.9478 & 0.9920 & 9.8183 
	%& 0.9825 & 19.0829 & 0.9554 & 35.0862 & 0.9272 & 45.4791 & 0.7638 & 0.8033 \\
	%\RankNet & 0.9987 & 2.9867 & 0.9978 & 4.9602 & 0.9937 & 9.7928 
	%& 0.9820 & 19.0493 & 0.9549 & 34.6926 & 0.9245 & 45.1706 & 0.7647 & 0.8013 \\
	\RankNet & 0.9978\rlap{*}  & 0.9987\rlap{*} & 2.9867\rlap{*} & 0.9978\rlap{*} & 4.9602 & \textbf{0.9937}\rlap{*} & 9.7928 
	& 0.9820 & 19.0493 & 0.9549 & 34.6926 & 0.9245 & 45.1706 \\ % & 0.7647 & 0.8013 \\
	\RankNet & 0.9978 & 0.9984 & 2.9824 & 0.9971 & \textbf{4.9630}\rlap{*} & 0.9926 & 9.7874
	& 0.9813 & 18.9579 & 0.9523 & 34.7077 & 0.9224 & 44.9721 \\ % & 0.7652 & 0.7971 \\
	%\RankNet & 0.9987 & 2.9867 & 0.9978 & 4.9602 & 0.9937 & 9.7928 
	%& 0.9820 & 19.0493 & 0.9549 & 34.6926 & 0.9245 & 45.1706 & 0.7647 & 0.8013 \\
	\RankNet & 0.9933 & 0.9963 & 2.9798 & 0.9954 & 4.9321 & 0.9910 & 9.8218\rlap{*} 
	& 0.9818 & 19.0944 & 0.9560 & 34.7844 & 0.9259 & 45.3864 \\% & 0.7621 & 0.8031 \\
	\RankNet & 0.9978 & 0.9984 & 2.9779 & 0.9962 & 4.9563 & 0.9931 & 9.8055 
	& \textbf{0.9828}\rlap{*} & 19.1335 & 0.9569 & 34.7795 & 0.9263 & 45.1717  \\ %& 0.7601 & 0.8021 \\
	\RankNet & 0.9978 & 0.9984 & 2.9803 & 0.9961 & 4.9565 & 0.9919 & 9.8038 
	& 0.9822 & {19.1363}\rlap{*} & 0.9557 & 34.6844 & 0.9249 & 45.3025 \\% & 0.7620 & 0.8030 \\
	\RankNet & 0.9933 & 0.9969 & 2.9822 & 0.9958 & 4.9432 & 0.9917 & 9.8179 
	& 0.9821 & 19.1201 & 0.9570\rlap{*} & 34.9531\rlap{*} & 0.9273\rlap{*} & 45.4070 \\ %& 0.7609 & 0.8026 \\
	%\RankNet & 0.9987 & 2.9777 & 0.9963 & 4.9478 & 0.9920 & 9.8183 & 0.9825 & 19.0829 & 0.9554 & 35.0862 & 0.9272 & 45.4791 & 0.7638 & 0.8033 \\
	%\RankNet & 0.9969 & 2.9822 & 0.9958 & 4.9432 & 0.9917 & 9.8179 & 0.9821 & 19.1201 & 0.9570 & 34.9531 & 0.9273 & 45.4070 & 0.7609 & 0.8026 \\
	\RankNet & 0.9978 & 0.9980 & 2.9756 & 0.9956 & 4.9432 & 0.9912 & 9.8008 
	& 0.9815 & 19.0667 & 0.9555 & 34.9568 & 0.9259 & 45.5265\rlap{*} \\%& 0.7641 & 0.8031 \\
	%\RankNet & 0.9987 & 2.9799 & 0.9970 & 4.9454 & 0.9921 & 9.7862 & 0.9801 & 18.7335 & 0.9397 & 32.9179 & 0.9032 & 42.1159 & \textbf{0.7797}\rlap{*} & 0.7955 \\
	%\RankNet & 0.9963 & 2.9803 & 0.9951 & 4.9392 & 0.9913 & 9.8202 & 0.9816 & 19.1146 & 0.9559 & 34.9911 & 0.9270 & 45.4015 & 0.7620 & 0.8039\rlap{*} \\
	\hline
	%%
	%\ListNet & 0.9987 & 2.9764 & 0.9962 & 4.9435 & 0.9920 & 9.7889 & 0.9810 & 18.9934 & 0.9543 & 35.0933 & 0.9267 & 45.6079 & 0.7564 & 0.8105 \\
	%\ListNet & 0.9987 & 2.9910 & 0.9979 & 4.9454 & 0.9921 & 9.7816 & 0.9809 & 19.0190 & 0.9546 & 35.0102 & 0.9260 & 45.2894 & 0.7547 & 0.8098 \\
	\ListNet & {0.9978}\rlap{*} & {0.9987}\rlap{*} & \textbf{2.9910}\rlap{*} &\textbf{ 0.9979}\rlap{*} & 4.9454 & 0.9921 & 9.7816 
	& 0.9809 & 19.0190 & 0.9546 & 35.0102 & 0.9260 & 45.2894 \\% & 0.7547 & 0.8098 \\
	\ListNet & 0.9978 & 0.9987 & 2.9846 & 0.9974 & 4.9587\rlap{*} & 0.9930\rlap{*} & 9.7969 
	& 0.9813 & 19.0486 & 0.9554 & 35.0682 & 0.9272 & 45.4353 \\% & 0.7550 & 0.8096 \\
	%\ListNet & 0.9987 & 2.9846 & 0.9974 & 4.9587 & 0.9930 & 9.7969 & 0.9813 & 19.0486 & 0.9554 & 35.0682 & 0.9272 & 45.4353 & 0.7550 & 0.8096 \\
	\ListNet & 0.9978 & 0.9972 & 2.9671 & 0.9943 & 4.9282 & 0.9903 & \textbf{9.8222}\rlap{*} 
	& 0.9812 & 19.0471 & 0.9553 & 34.8769 & 0.9261 & 45.3130 \\ %& 0.7540 & 0.8086 \\
	\ListNet & 0.9978 & 0.9987 & 2.9781 & 0.9972 & 4.9523 & 0.9925 & 9.8141 
	& 0.9825\rlap{*} & 19.0499 & 0.9555 & 34.9783 & 0.9273 & 45.5252 \\ %& 0.7562 & 0.8103 \\
	\ListNet & 0.9978 & 0.9983 & 2.9803 & 0.9963 & 4.9524 & 0.9918 & 9.8034 
	& 0.9820 & 19.1342\rlap{*} & 0.9563 & 34.8742 & 0.9274 & 45.1957 \\%& 0.7515 & 0.8086 \\
	\ListNet & 0.9978 & 0.9980 & 2.9848 & 0.9965 & 4.9389 & 0.9917 & 9.7933 
	& 0.9814 & 19.1320 & {0.9571}\rlap{*} & 35.0849 & 0.9285\rlap{*} & 45.4854 \\%& 0.7534 & 0.8099 \\
	\ListNet & 0.9933 & 0.9967 & 2.9695 & 0.9941 & 4.9308 & 0.9897 & 9.7908 
	& 0.9802 & 19.0805 & 0.9548 & {35.1009}\rlap{*} & 0.9271 & 45.5309 \\% & 0.7566 & 0.8100 \\
	%\ListNet & 0.9980 & 2.9848 & 0.9965 & 4.9389 & 0.9917 & 9.7933 & 0.9814 & 19.1320 & 0.9571 & 35.0849 & 0.9285 & 45.4854 & 0.7534 & 0.8099 \\
	\ListNet & 0.9978 & 0.9984 & 2.9824 & 0.9970 & 4.9499 & 0.9924 & 9.8095 
	& 0.9824 & 19.0410 & 0.9560 & 35.0411 & 0.9278 & 45.6343\rlap{*} \\% & 0.7559 & 0.8107 \\
	%\ListNet & 0.9974 & 2.9845 & 0.9963 & 4.9392 & 0.9919 & 9.7958 & 0.9809 & 19.0204 & 0.9549 & 35.0567 & 0.9268 & 45.5649 & 0.7573\rlap{*} & 0.8107 \\
	%\ListNet & 0.9984 & 2.9761 & 0.9962 & 4.9521 & 0.9921 & 9.7942 & 0.9815 & 19.0367 & 0.9551 & 35.0977 & 0.9272 & 45.5432 & 0.7563 &\textbf{ 0.8110}\rlap{*} \\
%	\hline
%	\ListNetCLA   & \textbf{1.0000}\rlap{*} & \textbf{0.9993}\rlap{*} & 2.9780 & 0.9965 & 4.9439 & 0.9911 & 9.7813 & 0.9803 & 19.0233 & 0.9551 & 34.8607 & 0.9254 & 45.2412 \\
%	\ListNetCLA   & 0.9978 & 0.9987 & 2.9824\rlap{*} & 0.9971\rlap{*} & 4.9453 & 0.9918 & 9.7945 & 0.9806 & 19.0163 & 0.9548 & 34.6270 & 0.9244 & 44.4960 \\
%\ListNetCLA   & 1.0000 & 0.9989 & 2.9760 & 0.9963 & 4.9480\rlap{*} & 0.9913 & 9.7828 & 0.9800 & 19.0009 & 0.9534 & 34.7735 & 0.9238 & 45.3510 \\
%\ListNetCLA   & 0.9978 & 0.9987 & 2.9821 & 0.9966 & 4.9435 & 0.9919\rlap{*} & 9.7812 & 0.9809 & 19.0262 & 0.9551 & 34.9057 & 0.9255 & 45.3877 \\
%\ListNetCLA   & 0.9978 & 0.9984 & 2.9737 & 0.9955 & 4.9433 & 0.9915 & 9.8128\rlap{*} & 0.9812\rlap{*} & 19.0126 & 0.9554\rlap{*} & 34.9533 & 0.9260 & 45.4187 \\
%\ListNetCLA   & 0.9978 & 0.9987 & 2.9713 & 0.9959 & 4.9413 & 0.9907 & 9.7816 & 0.9803 & 19.0704\rlap{*} & 0.9551 & 34.8866 & 0.9255 & 45.2965 \\
%\ListNetCLA   & 0.9978 & 0.9987 & 2.9756 & 0.9961 & 4.9373 & 0.9905 & 9.7812 & 0.9799 & 19.0464 & 0.9550 & 34.9702\rlap{*} & 0.9260\rlap{*} & 45.2266 \\
%\ListNetCLA   & 0.9978 & 0.9980 & 2.9672 & 0.9953 & 4.9304 & 0.9899 & 9.7839 & 0.9797 & 19.0274 & 0.9547 & 34.8758 & 0.9250 & 45.4837\rlap{*} \\
\hline
\SelNet &  \textbf{1.0000}\rlap{*} & 0.9986\rlap{*} & 2.9684 & 0.9940 & 4.8892 & 0.9855 & 9.7141 & 0.9770 & 19.1625 & 0.9563 & 35.1185 & 0.9267 & 45.6809  \\
\SelNet & 0.9978 & 0.9970 & 2.9763\rlap{*} & 0.9948 & 4.9291 & 0.9899\rlap{*} & 9.7853\rlap{*} & 0.9809\rlap{*} & 19.2005 & 0.9584 & 35.0994 & 0.9282 & 45.6769  \\
\SelNet & 0.9957 & 0.9975 & 2.9740 & 0.9951\rlap{*} & 4.9397\rlap{*} & 0.9891 & 9.7456 & 0.9803 & 19.2045 & \textbf{0.9585}\rlap{*} & 35.1140 & 0.9283\rlap{*} & 45.7155  \\
\SelNet & 0.9734 & 0.9851 & 2.9001 & 0.9805 & 4.8632 & 0.9784 & 9.7216 & 0.9744 & \textbf{19.2115}\rlap{*} & 0.9547 & 35.0343 & 0.9254 & 45.6236  \\
\SelNet & 0.9957 & 0.9960 & 2.9626 & 0.9934 & 4.9324 & 0.9889 & 9.7801 & 0.9801 & 19.1603 & 0.9577 & \textbf{35.1652}\rlap{*} & 0.9276 & 45.7312  \\
\SelNet & 0.9317 & 0.9575 & 2.8031 & 0.9545 & 4.6600 & 0.9444 & 9.1951 & 0.9335 & 18.3418 & 0.9198 & 34.9590 & 0.8991 & 45.7664\rlap{*}  \\
%\hline
%\SelNetCLA & 0.9868\rlap{*} & 0.9921\rlap{*} & 2.9304\rlap{*} & 0.9855\rlap{*} & 4.8364\rlap{*} & 0.9753\rlap{*} & 9.5591\rlap{*} & 0.9638\rlap{*} & 18.8122\rlap{*} & 0.9435\rlap{*} & 34.7920 & 0.9159\rlap{*} & 45.5440\rlap{*} \\
%\SelNetCLA & 0.9661 & 0.9791 & 2.8772 & 0.9740 & 4.7928 & 0.9661 & 9.5022 & 0.9569 & 18.7603 & 0.9392 & 34.9346\rlap{*} & 0.9136 & 45.5393 \\
	\bottomrule
	
	\end{tabular}

	\begin{tablenotes}
        \setlength\labelsep{0pt}
		\item The performances of the best performing model are in bold. 
		* indicates the best observed performance in a metric for a given model. 
		%$\dagger$ indicates that the model performs significantly better compared to \cclerank
		%according to a Wilcoxon signed rank test with Bonferroni correction 	at 5\% significance level.
		\par
	\end{tablenotes}

\end{threeparttable}
\end{table}
